NViST: In the Wild New View Synthesis from a Single Image with Transformers

We propose NViST, a transformer-based model for efficient and generalizable novel-view synthesis from a single image for real-world scenes. In contrast to many methods that are trained on synthetic data, object-centred scenarios, or in a category-specific manner, NViST is trained on MVImgNet, a large-scale dataset of casually-captured real-world videos of hundreds of object categories with diverse backgrounds. NViST transforms image inputs directly into a radiance field, conditioned on camera parameters via adaptive layer normalisation. In practice, NViST exploits fine-tuned masked autoencoder (MAE) features and translates them to 3D output tokens via cross-attention, while addressing occlusions with self-attention. To move away from object-centred datasets and enable full scene synthesis, NViST adopts a 6-DOF camera pose model and only requires relative pose, dropping the need for canonicalization of the training data, which removes a substantial barrier to it being used on casually captured datasets. We show results on unseen objects and categories from MVImgNet and even generalization to casual phone captures. We conduct qualitative and quantitative evaluations on MVImgNet and ShapeNet to show that our model represents a step forward towards enabling true in-the-wild generalizable novel-view synthesis from a single image. Project webpage: https://wbjang.github.io/nvist_webpage.

==> camera_ready/reviewer_reviews.tex <==

(AC)

Decision: Accept
Comment:
The paper received diverging reviews (WA, B, WR) in the initial phase. The authors kindly provided a detailed rebuttal addressing reviewers' concerns. There was an extensive discussion amongst reviewers in the post-rebuttal stage. The two reviewers updated their ratings from WA-to-Accept and B-to-WA. The third reviewer is still not convinced (and have kept their score) about the novelty of the proposed method and its positioning in context with concurrent methods (some of them being under review at the time of submission of this paper).

The AC went through the paper and closely checked the points discussed by the reviewers. After a close observation, the AC agrees with the two positive reviewers on the merits of accepting this paper. However, the authors are advised to add various quantitative and qualitative analysis in the main paper. This can be done by reducing a few qualitative analysis in the current version and moving a few of these in the supplementary material.

The decision is also verified by the AC triplet.


(R1)
Paper Summary:
The authors propose a method for novel view synthesis from a single image using radiance fields as the rendering principle. The authors leverage a pre-trained vision transformer (ViT) coupled with an attention mechanism over the encoded feature tokens and output tokens refined during training. The camera parameters are also inputs in this step using adaptive layer normalization. The result of these operation is then encoded as a radiance field using the Vector-Matrix (VM) representation of [11], which then can be used for volume rendering using the standard NeRF methodology of [40] to obtain color and density at every point. The method is trained on a subset of MVImgNet as well as ShapeNet-SRN, and the authors report experimental results on various settings, including out of distribution images.

Paper Strengths:
Using a ViT instead of a CNN for the feature extraction step makes sense to me, as they are able to better capture global information and enrich local patches with it.
Using a set of output tokens has the advantage that the network can learn to establish an association between features and given locations in the neural volume, though I wonder what the actual impact of this design choice is, that is, how would the method perform if the feature tokens were passed directly (e.g. by only using self-attention) to the MLP?
The authors use relative poses with respect to the scene instead of object-centric ones, which is a more challenging setup.
Both the quantitative and qualitative results show the effectiveness of this approach, and its generalization capabilities.
Paper Weaknesses:
Some of the claimed contributions are in my opinion not completely novel:

L. 088: "Efficient inference as it only needs one feed-forward pass": PixelNeRF also operates in this setting.
L. 089 "NViST only requires relative pose [...] and does not require a canonicalized dataset": The same applies to any method that uses a dataset where objects are not centered. To my knowledge PixelNeRF does the same for MVImgNet.
The authors claim that their method performs better on occluded parts, however, there is only some sparse qualitative evidence to assert this. It would be better in a final revision to highlight these or to include a quantitative analysis if possible.
It is not clear to me how large the range of novel views is based on the given experiments. Sometimes the motions are very small (e.g. Figure 4, microwave image). I wonder if the authors have a way of quantifying this range, and also, whether it depends on the complexity of the scene.
[Minor] I wonder if the authors have ablated the importance of using the camera parameters in the transformer decoder.
[Minor]: I wonder if the authors could explain how the output tokens are initialized. I would assume randomly, but it would be good to clarify.
[Minor]: The matrices used in the VM representation are denoted by 
. However, this symbol is also used in L. 274 to denote positional encodings, and once more in Eq. 2 as input to the 
 MLP. I would suggest the authors to update the notation to avoid this ambiguity.
Overall Recommendation: 4: weak accept
Justification For Recommendation And Suggestions For Rebuttal:
I am not an expert in this particular field, so I am looking forward to the reviews from the rest of my peers. However, the approach taken by the authors and the different design choices make sense to me. Using ViT and translating the processed tokens to a NeRF VM representation seems appropriate to model occlusions in the scene and to have a richer volume representation. Despite having noted some concerns in the weaknesses section, I think overall this draft is a solid submission based on my knowledge of the field, and thus vote WA.

Confidence Level: 4: The reviewer is confident but not absolutely certain that the evaluation is correct.
Final Rating: 5: Accept
Final Rating Justification:
Based on the discussion with the rest of the reviewers, I think that the paper has a few issues, such as:

Lack of comparison with diffusion-based approaches, which seem to be competitive with this method, such as "NeRDi: Single-View NeRF Synthesis with Language-Guided Diffusion as General Image Priors". As other reviewers pointed out, there are other works that can handle backgrounds, though to my knowledge they have not been published at peer-reviewed venues yet, so I do not think they should carry weight in the discussion as per the guidelines.
Missing evaluations: The authors have already included new results in the rebuttal, so I would encourage them to improve upon this on the rebuttal, including more qualitative comparisons with recent art.
As an improvement to ViT-based methods to NVS, the design choices of the method make sense to me and empirically bring improvements over existing art.
Since my expertise on the field is somewhat limited, I would err on the side of the authors and not block publishing, as I see some aspects of this work to be beneficial to the community, though I would ask the AC to carefully review the discussion that we had and make a final decision based on the different issues that were raised.

(R2)

Paper Summary:
This paper propose a single-view novel view synthesis method which first convert input image to a neural radiance field representation (vector-matrix representation in this paper) by a transformer architecture. By volume rendering, the image at target view can be recovered. Compared to previous methods, the proposed method can be used in scene-level images and achieve good performance on a zero-shot new-view synthesis task on out-of-distribution scenes captured on a mobile-phone device.

Paper Strengths:
This paper is easily understood and achieve good performance. It can also be generalized to any type of images (object-level or scene-level.)

Paper Weaknesses:
Line 015- 016: "First, unlike most generative models that are trained in a category-specific manner". Currently, some diffusion-based methods, like Zero123 train on a general dataset.
Line 088: Efficient inference is not a contribution. Previous work no matter transformer-based (SRT: Scene Representation Transformer) or generative model (Zero123) can achieve this.
Figure 2. There are two cls tokens and feature tokens. what is the difference between them? As there is no operation in the figure between them.
Line 231, a reference needs to be added for vector-matrix representation ([11])
Section 3.2.1, this part is not clear, do you use the same way as Zero123?
Section 3.2.2, the ablation study should include the comparison of different pose conditioning strategy to show the effectiveness of the design.
Table 1. More baseline methods are needed. For this task, there are different types of methods (NeRF-based, Re-projection based and diffusion-based, and latent-based, please refer to Consistent-1-to-3: Consistent Image to 3D View Synthesis via Geometry-aware Diffusion Models). But only one NeRF-based method is included here.
Overall Recommendation: 3: borderline
Justification For Recommendation And Suggestions For Rebuttal:
see the Weaknesses part. For now, more ablation study and baseline methods are needed to make this paper complete.

Confidence Level: 4: The reviewer is confident but not absolutely certain that the evaluation is correct.
Final Rating: 4: Weak Accept
Final Rating Justification:
According to the above discussion, I vote for a weak accept

(R3)

Paper Summary:
The paper investigates single-view 3D reconstruction, introducing NViST, which uses a Vision Transformer (ViT) as its backbone. It takes an image to infer vector-matrix decomposition as a 3D representation, subsequently rendered into a novel image in a single feed-forward pass. The network is supervised using 2D images. NViST is benchmarked against PixelNeRF on MVImgNet and compared with several recent diffusion-based novel view synthesis works on ShapeNet-SRN. It outperforms PixelNeRF and shows comparable performance to recent diffusion model-based work. Qualitative comparisons are provided in the supplementary materials.

Paper Strengths:
Recent works tend to prioritize time-consuming, heavy test-time optimization. This work shifts the focus back to inference efficiency, employing a single feed-forward pass at inference time.
The quality of its results is comparable to that of recent works. Notably, some real-world capture results seem encouraging.
Paper Weaknesses:
Unclear takeaways. After reading the paper, I am unclear about the key contribution. The design choices are quite straightforward (ViT as backbone, predict sparse tensor as 3D representation, volumetric neural rendering). None of the design choices are highlighted in the text or are supported by ablation studies.
1.1 Recent competition in this field is unfortunately intense, with many similar works like LRM (a concurrent work) and VisionNeRF (a published work in WACV). These studies share a common framework: a single feed-forward pass, reprojection as supervision, a form of 3D representation, and volumetric rendering. To stand out, a paper should offer novel insights, justify intricate design choices, or demonstrate extraordinary empirical results. Respectfully, the current version of this paper seems to fall short of these criteria. I illustrate them in the following bullet points.

In terms of quality, the method surpasses PixelNeRF but shows similar quality and is quantitatively underperformed when compared with more recent work like VisionNeRF (Vision transformer for nerf-based view synthesis from a single input image, WACV2023). It's concerning to see this performance gap given the close relation in concept but differences in implementation.

There are no ablation studies to support the claim of design choices. For example, the authors highlight the transformers architecture as the decoder novel. Then multiple design choices of backbone are expected.

Currently all qualitative comparisons are in supplementary material. I’d suggest putting qualitative comparisons to the main paper.

The writing could be improved with further revisions. Here are some suggestions: 5.1 The method section lacks hierarchical structure, with details uniformly distributed, making it difficult to discern the underlying insights of the method designs. For instance, the introduction of the number of parameters is too detailed to appear in the 1st paragraph. 5.2 The organization of the related works section could be improved. Some paragraphs, such as those on implicit and grid-based representations, could be condensed under a 3D representations. Others, like SSL, seem less relevant. A comprehensive review of single-view 3D reconstruction is essential as it’s the main topic. Please see LRM for a good example.
5.3 an overview of the experiment section will be helpful. Sec4.2 and table 2 is parallel to sec 4.1.2 and table 1 so I would consider merging these two.

Overall Recommendation: 2: weak reject
Justification For Recommendation And Suggestions For Rebuttal:
The field of single-view 3D reconstruction is progressing rapidly, and it's great to see the emphasis on computational efficiency in this paper. However, it seems that the paper could benefit from more distinct takeaways to differentiate it from other recent and concurrent works (W1). More specifically, 1) the quality appears similar to what's been reported in recent papers (W2), 2) the writing could be much more polished (W5), and 3) some design choices in the paper seem to need further justification (W3-4).

Confidence Level: 5: The reviewer is absolutely certain that the evaluation is correct and very familiar with the relevant literature.
Final Rating: 2: Weak Reject
Final Rating Justification:
I appreciate the authors for their responses. I regret any unintended offense caused by my use of the term "underperform“. I’ll explain it in 1.1.

Following extensive reviewer discussions, consensus may not be fully reached. However, I maintain my suggestion for another round of review prior to acceptance due to several notable issues that warrant further consideration.

Novelty issue (weakness 1 in my original review). Technical-wise, all of the components exists while the combination does not lead to significant empirical contribution. This is not the case that “all tricks combines shows something previously infeasible”. Prior works that also incorporate background [1-5] exist (some of them [1,4,5] are arxiv but they are from the last submission cycle, not recent). Theose prior works are also not acknowledged.

1.1. NiVT indeeds performs similar to prior work (VisionNeRF, WACV23) on SN. In the rebuttal, the authors show that visionNeRF cannot handle MVImgNet w background. But I believe the curent sota quality[1-5] surpass the current version of NViST. Notably, they show 360 views, whereas NViST only shows views close to the original view, which may be perceived as less challenging.

Some ablation results in the rebuttal add more confusion. In their rebuttal replacing vector-matrix with triplane hurts the performance significantly. e.g. LPIPS goes up to 0.5. Note that they train their visionnerf that gets completely blurry results (Fig.1 in rebuttal) and the LPIPS is only 0.47. This is so counter-intuitive since both are low-rank decomposition. In the original VM paper, it says that "their representation (triplane) is similar to our VM factorization and can be seen as a special VM version that has constant vectors." So the result is very bizarre to me. This demands further justification.

While the authors show some comparison (w/ VisionNeRF on SN-SRN, w/ PixelNeRF on MVImgNet, later one more figure in the rebuttal), there is no qualitative comparison throughout the main paper.

Overall, Tthe paper is not well contextualized to prior works. One notable issue is that the current version misses an important paragraph of comparisons on single-view 3D reconstruction / novel-view synthesis, which is exactly what the paper does....

One could argue that several of these weaknesses might be addressed with simple solutions such as including an additional paragraph, incorporating comparisons to the main paper, rewriting certain sections, and double-checking ablations. However, when combined, these issues accumulate to a degree that, in my view, necessitates another round of review.

I'll defer to the AC for their judgment.

[1] GeNVS, https://arxiv.org/pdf/2304.02602.pdf

[2] NerDi, Deng et al, CVPR 2023, see their DTU result

[3] Diffusion w forward model,

[4] ViewFormer

[5] ZeroNVS
